Cost-Effective In-Context Learning for Entity Resolution: A Design Space Exploration

Entity resolution (ER) is an important data integration task with a wide spectrum of applications. The state-of-the-art solutions on ER rely on pre-trained language models (PLMs), which require fine-tuning on a lot of labeled matching/non-matching entity pairs. Recently, large languages models (LLMs), such as GPT-4, have shown the ability to perform many tasks without tuning model parameters, which is known as in-context learning (ICL) that facilitates effective learning from a few labeled input context demonstrations. However, existing ICL approaches to ER typically necessitate providing a task description and a set of demonstrations for each entity pair and thus have limitations on the monetary cost of interfacing LLMs. To address the problem, in this paper, we provide a comprehensive study to investigate how to develop a cost-effective batch prompting approach to ER. We introduce a framework BATCHER consisting of demonstration selection and question batching and explore different design choices that support batch prompting for ER. We also devise a covering-based demonstration selection strategy that achieves an effective balance between matching accuracy and monetary cost. We conduct a thorough evaluation to explore the design space and evaluate our proposed strategies. Through extensive experiments, we find that batch prompting is very cost-effective for ER, compared with not only PLM-based methods fine-tuned with extensive labeled data but also LLM-based methods with manually designed prompting. We also provide guidance for selecting appropriate design choices for batch prompting.

==> algorithms/coreset_selection.tex <==
\begin{algorithm}
    \caption{$CoresetSelection(M, D_u, f)$}\label{alg:coreset_selection}
    \begin{algorithmic}[1]
    \renewcommand{\algorithmicrequire}{ \textbf{Input:}}
    \REQUIRE collection of pairs $M$, unlabelled demo set $D_u$, nondecreasing value function $f$.
    \renewcommand{\algorithmicrequire}{ \textbf{Output:}}
    \REQUIRE selected demo subset $D_s$.
    
    \STATE $D_s \gets \varnothing$

    \WHILE{$f(D_s) \neq f(D_u)$}
        \STATE $d \gets \mathop{\arg\min}\limits_{d\in D_u} \frac{1}{f(D_s \cup \{d\})-f(D_s)}$
        \STATE $D_s \gets D_s \cup \{d\}$
    \ENDWHILE
    \end{algorithmic}
\end{algorithm}
    

==> algorithms/pair_packaging.tex <==
\begin{algorithm}
\caption{Greedy algorithm for Pair Packaging}\label{alg:pair_packaging}
\begin{algorithmic}[1]
\renewcommand{\algorithmicrequire}{ \textbf{Input:}}
\REQUIRE pair set $M$, similarity threshold $t_s$ and tokens threshold $T$.
\renewcommand{\algorithmicrequire}{ \textbf{Output:}}
\REQUIRE generated batches $B$.
\STATE $M^* \gets clustering(M)$
\STATE $B \gets \varnothing$
\WHILE{$M^* \neq \varnothing$}
    \STATE $p_r \gets get\_root(M^*)$
    \STATE $R \gets \{p_r\}$, $B' \gets \{\{p_r\},\}$
    \STATE $M^* \gets M^*-{p_r}$
    \FOR{$p$ in $M^*$}

        \IF{$tokens(B') + tokens(p) \geq T$}
            \STATE $break$
        \ENDIF

        \STATE $p_r^{-}, p_r^{+} \gets \mathop{\arg\min}\limits_{p_r\in R} \mathrm{sim}(p_r, p), \mathop{\arg\max}\limits_{p_r\in R} \mathrm{sim}(p_r, p)$
        \STATE $mi, ma \gets \mathrm{sim}(p_r^{-}, p), \mathrm{sim}(p_r^{+}, p)$
        
        \IF{$ma > 1-mi$ and $ma > t_s$}
            \STATE $B'(p_r^{+}) \gets B'(p_r^{+})+\{p\}$
            \STATE $M^* \gets M^*-\{p\}$
        \ELSIF{$ma \leq 1-mi$ and $1-ma < t_s$}
            \STATE $R \gets \{p_r^{-}\}$
            \STATE $B'(p_r^{-}) \gets \{\{p_r^{-}\},\}$
            \STATE $M^* \gets M^*-\{p\}$
        \ELSE 
            \STATE $continue$
        \ENDIF
    \ENDFOR

    \STATE $B \gets B\cup B'$
    
\ENDWHILE
\end{algorithmic}
\end{algorithm}

==> figure_tex/instance_batch_cover.tex <==
\begin{figure}[!t]
    \centering 
    \includegraphics[width=0.5\columnwidth]{plots/example_selection/instance_batch_covering.pdf}
    \caption{Instance for covering batch.}
    \label{fig:instance_batch_covering}
\end{figure}
